Multi-Target Emotional Voice Conversion With Neural Vocoders

Emotional voice conversion (EVC) is one way to generate expressive synthetic speech. Previous approaches mainly focused on modeling one-to-one mapping, i.e., conversion from one emotional state to another emotional state, with Mel-cepstral vocoders. In this paper, we investigate building a multi-target EVC (MTEVC) architecture, which combines a deep bidirectional long-short term memory (DBLSTM)-based conversion model and a neural vocoder. Phonetic posteriorgrams (PPGs) containing rich linguistic information are incorporated into the conversion model as auxiliary input features, which boost the conversion performance. To leverage the advantages of the newly emerged neural vocoders, we investigate the conditional WaveNet and flow-based WaveNet (FloWaveNet) as speech generators. The vocoders take in additional speaker information and emotion information as auxiliary features and are trained with a multi-speaker and multi-emotion speech corpus. Objective metrics and subjective evaluation of the experimental results verify the efficacy of the proposed MTEVC architecture for EVC.

==> __latexindent_temp.tex <==
@inproceedings{liu2018hccl,
  title={The HCCL-CUHK System for the Voice Conversion Challenge 2018},
  author={Liu, Songxiang and Sun, Lifa and Wu, Xixin and Liu, Xunying and Meng, Helen},
  booktitle={Proc. Odyssey 2018 The Speaker and Language Recognition Workshop},
  pages={248--254},
  year={2018}
}
